Verification for Reliable Product Lines

Many product lines are critical, and therefore reliability is a vital part of their requirements. Reliability is a probabilistic property. We therefore propose a model for feature-aware discrete-time Markov chains as a basis for verifying probabilistic properties of product lines, including reliability. We compare three verification techniques: The enumerative technique uses PRISM, a state-of-the-art symbolic probabilistic model checker, on each product. The parametric technique exploits our recent advances in parametric model checking. Finally, we propose a new bounded technique that performs a single bounded verification for the whole product line, and thus takes advantage of the common behaviours of the product line. Experimental results confirm the advantages of the last two techniques.

==> sections/CTMC.tex <==
\section{Continuous-Time Markov Chains}

==> sections/Implementation.tex <==
\section{Implementation}
\label{sec:Implementation}



==> sections/MotivatingRunningExample.tex <==
\section{Motivating Running Example}
\label{MotivatingRunningExample}

As a running example, we use a slightly changed version of the case study introduced in \cite{Classen2010}. The example refers to a product line that produces various vending machines. Figure \ref{example} shows the feature model for the product line. The general scenario is that a user inserts coins into the machine and receives some change. At this point, she may cancel the purchase or chooses a beverage, and the vending machine prepares and delivers it. As illustrated in the feature model, a vending machine may have capability to prepare tea, soda, or both. It may require a cash payment or may simply offer a free drink. Similarly, it may support a feature to add taste (e.g. lemon) to a beverage.

\begin{figure}[h]
\begin{center}
\includegraphics[width=8.0cm]{figure/Feature}
\caption{Feature model for the motivating example.}
\label{example}
\end{center}
\end{figure}

==> sections/TheProposedFramework.tex <==
\section{Featured Markov Reward Models}
\label{TheProposedFramework}

Nowadays, the satisfaction of non-functional requirements like reliability and energy consumption is an important challenge in software engineering. When combined with uncertainty (that is, randomness), their assessment becomes even more cumbersome. Depending on both the system and the property to verify, different kinds of models are used. In particular, Markov chains and Markov reward models are very popular. However, their analysis becomes harder as the size of the models grows. Furthermore, in an SPL with $n$ features, checking non-functional properties on every product variant requires the analysis of up to $2^n$ Markov models, that is, one for each product variant. Even though this number is reduced because of the constraints between the features, this enumerative approach is clearly infeasible in industrial context, where SPLs may include hundreds of variants. 

In order to reduce the verification effort, we propose a new approach for verifying SPLs. Our method relies on the definition of a new formalism, which results from the enrichment of Markov models with operators to express variability. From an instance of this formalism, we derive a parametric Markov model. We feed this model into a parametric model-checker that subsequently returns a rational (parametric) expression. We are then able to derive, for each variant of the SPL, the corresponding value of this expression. This way, we are able to assess the satisfaction of non-functional properties for the whole product line.

\subsection{Variability in Stochastic Systems}
We previously mentioned that Markov Reward Models (MRMs) are convenient for modeling non-functional properties in single systems. Since we are interested in SPL, we extend this formalism so that it can represent variability. We propose to equip MRMs with an explicit notion of features. %, in the same vein as the featured transition systems proposed by Classen \textit{et al.}~\cite{Classen2010}. 
Beforehand, it is essential to define how features may impact on a given system. In this paper, we consider that a feature can have the following effects.
\begin{itemize}
	\item[(1)] It can modify \emph{transition availability}, that is, it can add or remove transitions. This is useful to model that a feature can introduce new capabilities, functions, or components that augment the set of possible behaviors in the system.
	\item[(2)] It can alter \emph{probability distributions}. For example, a feature could model an optional component that increases the reliability of the global system.
	\item[(3)] It can change the \emph{reward} the system gets by reaching a given state. In the context of reliable systems and energy consumption, a feature improving the reliability of the system will more likely increase its total energy consumption.
\end{itemize}
For our new formalism to be appropriate, it has to be able to cope with these three types of variability. We briefly present how we will deal with them. In the next subsections, we illustrate and formalize the concepts we introduce below.

Variable transition availability has already been studied by Classen \textit{et al.} in the context of their work on featured transition systems~\cite{Classen2010, Classen2011}. In their second article~\cite{Classen2011}, they propose to label transitions with constraints on the features, called \emph{feature expressions}. Since feature expressions come down to Boolean functions, they are an intuitive but powerful construct to express variability. They also benefit from existing efficient representations (in particular, binary decision diagrams). We could make use of feature expressions in the current paper as well. However, this kind of variability is a particular case of the second one : if a transition cannot be executed, it means that it has an execution probability of zero.

Because features can modify the probability distribution of an MRM, the probability of a given transition is not known \textit{a priori} anymore. Hence, if a transition $t$ is subject to variations in its execution probability, we specify this probability with a parameter. We associate a \emph{probability profile} to the parameter that, for each valid product, defines a value for the parameter. By doing so, we have the potential to give distinct transition probabilities for every product. In reality, however, it is unlikely that all the transitions will receive a different probability value for every product. In a given model $M$, we call the probability profiles of $M$ the set of probability profiles that determine the value of the parameters. Note that all these profiles must satisfy the probability axioms. In particular, the sum of the execution probability of the outgoing transitions in a given state must be equal to 1. The profiles must thus be consistent to ensure the satisfaction of these axioms.

We use a similar construct for modeling the impact of variability on reward. We define \emph{reward profiles} that provide each state with a function that determines, for each combination of features, the actual value of the reward earned by reaching this state. Once again, it is very unlikely that every product gives rise to a different reward value. Nevertheless, we want our models to be generic enough to consider these worst cases. The above two constructs lead us to our new formalism, \emph{Featured Markov Reward Models}~(FMRMs), which are usual MRMs equipped with probability and reward profiles.

\subsection{Introductory Example}
\begin{figure}
	\begin{center}
		\includegraphics[scale=0.55]{figure/fd.pdf}
	\end{center}
	\caption{Feature diagram of the wiper system.}
	\label{fig:fd}
\end{figure}
Before we provide FMRM with a formal syntax and semantics, we present its modeling capabilities through an introductory example. Inspired by Gruler \textit{et al.}~\cite{Gruler2008}, we consider a wiper systems SPL whose behavior is determined according to (stochastic) falls of rain. The feature diagram modeling the variability in this SPL is given in Figure~\ref{fig:fd}. A product of the SPL has two components : a sensor and a wiper. The sensor is either normally sensitive ($std$) or very sensitive ($very$). The wiper has either one speed $(spd1)$ or two speeds ($spd2$). The optional feature $economic$ ($eco$) reduces the overall energy consumption of the wiper. According to the semantics of feature diagram we have given in Section~\ref{sec:spl-modeling}, this SPL is composed of 8 products.

Before we illustrate how we model the stochastic behavior of this SPL, let us first consider the product with standard sensor and one speed.  An MRM modeling its behavior is given in Figure~\ref{fig:product}. The system first start in \texttt{off} state. Then, if it rains (0.8 probability), the system moves to the $on$ state, meaning that the wiper system is activated. On the contrary, if no rain falls then the system remains in the \texttt{off} state (0.2 probability). Once in the \texttt{on} state, either it continues to rain and the system remains in state \texttt{on} (0.8 probability) or it stops raining and the system moves to the \texttt{end} state (0.2 probability). The \texttt{end} state is absorbing and marks the end of our scenario. In this case, the reward models the energy consumption of the wiper between two rain falls. The wiper consumes three energy units in state \texttt{on} and zero in the others.

%\begin{figure}
%	\begin{center}
%		\subfigure[Product with standard sensor and one speed.]{
%		\includegraphics[scale=0.70]{figure/mrm1.pdf}
%			\label{fig:product}
%		}\\
%		\subfigure[The above product plus the feature $spd2$.]{
%		\includegraphics[scale=0.70]{figure/mrm-feature.pdf}
%			\label{fig:spd2}
%		}\\
%		\subfigure[Complete model of the SPL.]{
%		\includegraphics[scale=0.70]{figure/fmrm.pdf}
%			\label{fig:fmrm}
%		}\\
%	\end{center}
%	\caption{Models of the wiper system.}
%	\label{fig:wipermodels}
%\end{figure}

\begin{figure}
	\begin{center}
		\includegraphics[scale=0.70]{figure/mrm1.pdf}
	\end{center}
	\caption{Wiper system with standard sensor and one speed.}
	\label{fig:product}
\end{figure}


Let us now describe the effect of all the optional and alternative features on that model. The feature $spd2$ allows the wiper to run in a higher speed mode whenever the rain is considered as heavy. Thus, when this features is enabled the wiper can enter a \texttt{fast} state in case of heavy rain. In this state, the wiper consumes six energy units. Heavy rain occurs with a probability of 0.3, whereas light rain has an occurrence probability of 0.5. It means that the feature $spd2$ reduces the probability of transition to state \texttt{on} from 0.8 to 0.5. The resulting model is shown in Figure~\ref{fig:spd2}. 
\begin{figure}
	\begin{center}
		\includegraphics[scale=0.70]{figure/mrm-feature.pdf}
	\end{center}
	\caption{Wiper system with optional $spd2$ feature.}
	\label{fig:spd2}
\end{figure}
Each time a probability value is subject to variations, we replace it with a parameter and we associate it with a probability profile that determines its actual value according to the enabled features. Two parameters are part of this model. The first, $\alpha$, determines the probability that the wiper goes to state \texttt{on}. Without the feature $spd2$, the wiper necessarily moves to this state whenever it rains, that is, with a probability of $0.8$. On the contrary, if the feature is enabled then the wiper can either move to state \texttt{on} in case of light rain (with a probability of 0.5) or to the state \texttt{fast} in case of heavy rain (probability of 0.3). Hence, the parameter profile of $\alpha$ and $\beta$ is given by
\begin{align}
\alpha &= \left \lbrace 
		\begin{array}{ll}
			0.8, & \lnot spd2\\
			0.5, & spd2,
		\end{array}
\right . \\
\beta &= \left \lbrace 
		\begin{array}{ll}
			0, & \lnot spd2\\
			0.3, & spd2.
		\end{array}
\right .
\end{align}
In the above equations, we do not explicitly define the value of a parameter for every product. Instead, we use feature expressions to easily specify a parameter value common among several products. To further increase the conciseness of the specification, we can define $\beta$ as $\beta = 0.8 - \alpha$. Also, note that we could have written $spd1$ instead of $\lnot spd2$ to specify the value of the parameters when the wiper system has one speed. However, given that $spd1$ and $spd2$ share a XOR relationship and that every product has exactly one of these features, we only need information about one of them to determine the presence or absence of the other. We will proceed similarly for the features $std$ and $very$.

The feature $very$ rises the sensitivity of the wiper sensor. It means that rain falls that were previously considered as light may now be perceived as heavy. The resulting model of the wiper SPL is shown in Figure~\ref{fig:fmrm}. The probability of reaching state \texttt{on} (resp. \texttt{fast}) is decreased (resp. increased) when this feature is enabled. The probability profile of $\alpha$ and $beta$ is then modified as follows: 
\begin{align}
\alpha &= \left \lbrace 
		\begin{array}{ll}
			0.8, & \lnot spd2\\
			0.5, & spd2 \land \lnot very \\
			0.2, & spd2 \land very,
		\end{array}
\right . \\
\beta &= \left \lbrace 
		\begin{array}{ll}
			0, & \lnot spd2\\
			0.3, & spd2 \land \lnot very\\
			0.6, & spd2 \land very.
		\end{array}
\right .
\end{align}
Moreover, the execution probabilities of the outgoing transitions of \texttt{fast} are not constant anymore; they also depend on the feature. The probability of the self-loop in \texttt{fast} is determined according to the same probability profile as the other transitions that reach this state, that is, the profile of $\beta$. On the other hand, the probability of the transition from \texttt{fast} to \texttt{on} is determined according to $\alpha$. %, except that the feature $spd2$ is known to be enabled (otherwise, the system would not have been able to reach state \texttt{fast}). 
Note that $very$ is meaningful if and only if the feature $spd2$ is enabled as well. Otherwise, the wiper would not have to distinguish between light and heavy rain, since it has only one speed nevertheless.

Finally, the purpose of the feature $eco$ is to reduce energy consumption by a factor of 1.5. The feature thus modifies the reward of the states, but leaves the probability values unchanged. Consequently, we equip each state with a reward profile that provides the reward values obtained by reaching this state. The profiles of \texttt{off} and \texttt{end} specify the value 0 whatever the enabled features. For states \texttt{on} and \texttt{fast}, they are given by
\begin{align}
R(\texttt{on}) &= \left \lbrace 
		\begin{array}{ll}
			3, & \lnot eco\\
			2, & eco,
		\end{array}
\right . \\
R(\texttt{fast}) &= \left \lbrace 
		\begin{array}{ll}
			6, & \lnot eco\\
			4, & eco.
		\end{array}
\right .
\end{align}
 
\begin{figure}
	\begin{center}
		\includegraphics[scale=0.70]{figure/fmrm.pdf}
	\end{center}
	\caption{Complete model of the wiper SPL.}
	\label{fig:fmrm}
\end{figure} 
 
\subsection{Formal syntax and semantics}
\label{definitions}
In this subsection, we formalize the syntax of our new formalism and provide it with a semantics. We define FMRMs as follows.

\begin{definition}
An FMRM is a tuple $(S, E, \nu, P, d, \Pi, \Xi)$ where
\begin{itemize}
	\item $S$ is a countable, non-empty set of states;
	\item $E$ is a set of parameters;
	\item $\nu$ is a vector of size $| S |$ that records the initial probability distribution of every state;
	\item $P : S \times S \rightarrow [0,1] \cup E$ is the transition probability function, which assigns either a probability value of a parameter to every transition;
	\item $d = (N, \fdsem{d}\subseteq \mathcal{P}(N))$ is a feature diagram
%	\item $\gamma : S \times S \rightarrow (\{\top, \bottom\}^{| N |} \rightarrow \{\top, \bottom\})$ is the transition availability function that labels every transition with a feature expression;
	\item $\Pi : E \rightarrow (\fdsem{d} \rightarrow [0,1])$ is a total function called probability profile;
	\item $\Xi : S \rightarrow (\fdsem{d} \rightarrow \mathbb{R}^{+}_0)$ is a total function called reward profile.
\end{itemize}
\end{definition}
Note that any instance of FMRM must ensure the satisfaction of the usual \emph{probability axioms}. In particular, the sum of the probability of each random outcome must be equal to one. It implies that the sum of the initial probability of all the states must be one : $\sum_{s \in S} \nu(s) = 1$. For every state, the probability sum of its outgoing transition must be one as well. Since features can influence transition probabilities, this assertion must hold for all the valid products. The actual value of a parameter is thus determined according to the considered product and the probability profile $\Pi$. Formally, we must have
$$\forall s \in S \suchthat \forall p \in \fdsem{d} \suchthat \sum_{s' \in S} P'(s,s') = 1$$
where
$$P'(s,s') = \left \lbrace 
	\begin{array}{ll}
		P(s,s'), & P(s,s') \in [0,1],\\
		\Pi(\alpha, p),& P(s,s') = \alpha.
	\end{array}
	\right .$$
We call \emph{product-consistent} any FMRM that satisfies the above property. In the rest of this paper, we consider only product-consistent FMRMs.

One could argue that our definition is too general and can be drastically simplified under additional assumptions. For example, we could have assumed that when a given transition is not executable for a certain product, then its execution probability is redistributed uniformly between the other outgoing transitions of the current state. In this case,   we can spare ourselves the trouble of using parameters and the probability profile; the formalism would only require a probability value for every transition. Another simplification consists in associating a feature with a \emph{unique} parameter. It means that each time this feature can modify the behavior of the system, the corresponding transition has always the same execution probability. For instance, a cross-cutting feature that takes effect in very specific states and may result in a transition with a fixed probability of occurrence. In this case, we only need one parameter for every such variation point. Since the number of parameters decreases, the model is simplified.

However, whether or not these assumptions are valid depends only on the studied system. We want our modeling formalism to remain sufficiently generic so that it can be applied to a wide range of SPLs. Like usual Markov models, FMRM can be regarded as a framework and derived into simplified forms in very specific cases. Consequently, we will stick to the above definition.

An FMRM is a concise representation for a set of MRMs, that is, one per valid products. To retrieve the MRM corresponding to a given product $p$, we define a \emph{projection} operator\footnote{Classen \textit{et al.}~\cite{Classen2010} defined a similar operator for featured transition systems.} that extracts it from the FMRM. This operator consists in first replacing each parameter by the value determined by its probability profile and $p$, and then replacing each reward by the value given by the reward profile for $p$. 
%\begin{enumerate}
%	\item Set to 0 the execution probability of every transition that $p$ cannot execute.
%	\item Replace each parameter by the value determined to the probability profile and $p$.
%	\item Replace each reward by the value given by the reward profile for $p$.
%\end{enumerate}
For example, the projection of the FMRM shown in Figure~\ref{fig:fmrm} onto the product with standard sensor, one speed, and no economic function is the MRM given in Figure~\ref{fig:product}. Formally, we define the projection as follows.
\begin{definition}
\label{def:proj}
	The projection of an FMRM $fm = (S, E,$ $\nu,$ $P, d,$ $\Pi, \Xi)$ onto a product $p \in \fdsem{d}$, noted, $fm \reduc{p}$ is the MRM $(S, \nu, P', R)$ where $\forall s, s' \in S$ we have
	\begin{align}
		\label{eq:proj-p}
		P'(s,s') &=  \left \lbrace
			\begin{array}{ll}
%			0, & p \not\in \sem{\gamma(s,s')},\\
				P(s,s'), & P(s,s') \in [0,1],\\
				\Pi(\alpha, p), & P(s,s') = \alpha,
			\end{array} \right . \\
		R(s) &= \Xi(s,p).
	\end{align}
\end{definition}
Then, we define the semantics of an FMRM $fm$ as a function $\sem{fm}_{FM}$ that associates a valid product with the semantics of its projected MRM, that is, $\forall p \in \fdsem{d} \suchthat \sem{fm}_{FM}(p) = \sem{fm \reduc{p}}_{MR}$ where $\sem{.}_{MR}$ denotes the usual semantics of a Markov reward model.

Note that as MRM is an extension of Markov chains, our definition of FMRM encapsulates the notion of one would call ``Featured DTMC''. It means that all the results presented in this paper, including the verification procedures presented and the next subsection, are applicable to SPLs modelled as DTMCs. In this case, features influence the availability of transitions and their execution probability.

\subsection{Verification of non-functional properties}
\label{sec:verification}
Markov models and more particularly MRMs are convenient for modeling stochastic and non-functional aspects of individual systems. By providing FMRM with a semantics in terms of MRM, we obtain a new formalism that combines the expressivity of MRMs with three types of variability representations. This way, we fill an important gap in SPL modeling.

Still, we have to provide methods for verifying such models. In this paper, we are interested in PCTL and Reward-based properties. For instance, a Reward-based property desired for the wiper SPL is ``what is the mean energy consumed by the wiper system when reaching the \texttt{end} state''. We want to assess the satisfaction of such properties for all the valid products of a given SPL.

Given its semantics, we can check an FMRM against this property using standard MRM verification algorithms. This procedures, called \textbf{enumerative}, consists in computing the projection of the FMRM to all products, and then model checking each projection individually. This method, however, does not benefit from the commonalities between the products. In consequence, we propose another approach based on \textbf{parametric} model checking of Markov models.

Let us observe that according to Definition~\ref{def:proj}, the projection of an FMRM onto a product is a MRM without parameter. It means that only the features of the products have to be known to determine the possible values of the parameters. Hence, we can convert an FMRM into a parametric MRM where the parameters are the features, and reuse existing methods for model checking parametric MRMs. In this subsection, we discuss how we can achieve this conversion. Since variability manifests itself in two forms, we show that each of these boils down to adding parameters to the Markov models.

%The first form of variability impacts on transitions availability. Let $\gamma(s,s')$ be the feature expression characterizing the availability of the transition from $s$ to $s'$. Then, for all products $p' \not\in \sem{\gamma(s,s')}$, $p'$ cannot execute the transition. In other words, the probability of the transition is 0 for these products. Remember that we define a product as a set of features. Since features can be regarded as Boolean variables, we can express the above property by transforming $\gamma(s,s')$ into an arithmetic parametric expression. A given assignation of features makes this expression equal to zero (resp. one) if and only if the corresponding product cannot (resp. can) execute the transition. A parametric expression  $\epsilon(e)$ is derived from a feature expression $e$ according to the following rules :
%$$\epsilon(e) = \left\lbrace 
%	\begin{array}{ll}
%		min(\epsilon(e_1), \epsilon(e_2)), & e = e_1 \land e_2,\\
%		max(\epsilon(e_1), \epsilon(e_2)), & e = e_1 \lor e_2,\\
%		1 - f, & e = \lnot f,\\
%		f, & e = f.
%	\end{array}
%\right .$$
%Once this parametric expression is derived, we replace $P(s,s')$ by $\epsilon(e) \times P(s,s')$. For a given product $p$ the execution probability of the transition is thus $0$ if $p \not\in \sem{\gamma(s,s')}$ and $P(s,s')$ otherwise. This corresponds exactly to Equation~\ref{eq:proj-p} in Definition~\ref{def:proj}. The transformation thus preserves the semantics of the original FMRM.

The first type of variability we encounter in FMRM concerns the probability distribution. It is represented by the aforementioned probability profile. We previously described a probability profile as a function $\Pi$ that associates a parameter $\alpha$ with a function noted $\Pi(\alpha)$ such that $\Pi(\alpha)$ gives a value to $\alpha$ for every product. We can represent $\Pi(\alpha)$ as a parametric expression where the parameters are the features. For this purpose, we sum up the values of $\alpha$ can take, weighted by a parametric expression designating the corresponding product. We denote by $\epsilon(p)$ the parametric expression corresponding to the product $p$. Let $\{f_1, \dots, f_k\} \in \mathcal{P}(N)$ be a product and $\{f'_1, \dots, f'_j\}$ the set of features that this product does not have. Then, $\epsilon(p)$ is given by
\begin{align}
	\epsilon(p) &= b_1 \times \dots \times b_k \times b_{k+1} \times \dots \times b_{k+j},\\
	b_i &= \left\lbrace 
	\begin{array}{ll}
		f_i, & i = 1 \dots k,\\
		1 - f'_{i-k}, & i = k+1 \dots k+j
	\end{array}
	\right .
\end{align}
Intuitively, this parametric expression is equal to 1 if we assign the value 1 to all the features of $p$ and the value 0 to all the others. For any other assignation, the expression is equal to 0.

Using the above construction, we represent the function $\Pi(\alpha)$ as the parametric expression
\begin{equation}
\label{eq:fparam}
	\sum_{p_i \in \mathcal{P}(N)} \epsilon(p_i) \times \Pi(\alpha,p_i).
\end{equation} 
When considering a particular product $p$, every term of this sum except one is equal to 0; the remaining term is equivalent to $\Pi(\alpha,p)$. Note that if several products share the same value for $\alpha$, we can drastically simplify the above sum. In particular, if the value of $\alpha$ depends only on a feature $f$, then we can rewrite Equation~\ref{eq:fparam} as $f \times \alpha_1 + (1 - f) \times \alpha_0$ where $\alpha_1$ (resp. $\alpha_0$) is the value of $\alpha$ when the feature $f$ is enabled (resp. disabled). This way of reducing the complexity of parameters profile has already been illustrated in the previous subsection.

The second form of variability makes the reward earned through the execution of a transition depend on features as well. To cope with it, we use a technique similar to the previous one, that is, we define the reward of a given transition as a parametric expression over the set of features. We thus represent $\Xi(s)$ by the expression
\begin{equation}
\label{eq:freward}
	\sum_{p_i \in {\top, \bottom}^{|N|}} \epsilon(p_i) \times \Xi(s, p_i).
\end{equation} 
As for the previous case, we will often be able to write the above sum as a more concise expression.

By performing the above two transformations, we reduce FMRM verification to parametric MRM verification, where the parameters are all Boolean variables that model the presence or absence of features. In consequence, we are able to benefit from efficient parametric model-checkers like PARAM~\cite{Hahn2010} and the tool of Filieri \textit{et al.}~\cite{Filieri2011}. Given a parametric model, those tools return a rational expression containing parameters. In our context, the parameters are variables corresponding to the features. The expression represents the probability or the reward we seek. To determine the actual probability or reward of a given product, we simply replace, in the expression, each feature by 1 if it belongs to the product, or by 0 if it does not.

\begin{figure}
	\begin{center}
		\includegraphics[scale=0.56]{figure/pmrm.pdf}
	\end{center}
	\caption{Parametric model corresponding to the wiper systems SPL.}
	\label{fig:pmrm}
\end{figure} 

\textbf{Example}. We applied this methodology to the aforementioned wiper systems SPL. We first transformed the FMRM modeling this SPL into a parametric model. This operation yields the parametric MRM shown in Figure~\ref{fig:pmrm}. Then, we fed the model into the model checker of Filieri \textit{et al.}~\cite{Filieri2011}, which returned the rational expression
$$\frac{\begin{split}
				(-15*spd2*eco*very -15*spd2*eco + \\ 45*spd2*very +45*spd2 -40*eco +120)
			\end{split}}
		{8}.$$
According to the above formula, the product with a very sensitive sensor and two speeds consumes 26.25 energy units on average. If the economic feature is enabled as well, this amount is reduced to 17.5 units.
